Shuffle Private Linear Contextual Bandits

Differential privacy (DP) has been recently introduced to linear contextual bandits to formally address the privacy concerns in its associated personalized services to participating users (e.g., recommendations). Prior work largely focus on two trust models of DP: the central model, where a central server is responsible for protecting users sensitive data, and the (stronger) local model, where information needs to be protected directly on user side. However, there remains a fundamental gap in the utility achieved by learning algorithms under these two privacy models, e.g., $\tilde{O}(\sqrt{T})$ regret in the central model as compared to $\tilde{O}(T^{3/4})$ regret in the local model, if all users are unique within a learning horizon $T$. In this work, we aim to achieve a stronger model of trust than the central model, while suffering a smaller regret than the local model by considering recently popular shuffle model of privacy. We propose a general algorithmic framework for linear contextual bandits under the shuffle trust model, where there exists a trusted shuffler in between users and the central server, that randomly permutes a batch of users data before sending those to the server. We then instantiate this framework with two specific shuffle protocols: one relying on privacy amplification of local mechanisms, and another incorporating a protocol for summing vectors and matrices of bounded norms. We prove that both these instantiations lead to regret guarantees that significantly improve on that of the local model, and can potentially be of the order $\tilde{O}(T^{3/5})$ if all users are unique. We also verify this regret behavior with simulations on synthetic data. Finally, under the practical scenario of non-unique users, we show that the regret of our shuffle private algorithm scale as $\tilde{O}(T^{2/3})$, which matches that the central model could achieve in this case.

==> Shuffle Linear Bandit Arxiv/new_return.tex <==
Similar to existing work on differentially private bandits, in previous sections, we have assumed that all participating users are unique, i.e., each user participates in the protocol only at one round. A more practical scenario is that an user can contribute with her data at multiple rounds. For example, consider the mobile medical application described in the introduction. The cloud server can collect one particular user's data during multiple batches to track the effectiveness of its treatment plan over a period, and hence, use same user's data multiple times to update its recommendation algorithm. Motivated by this, we provide privacy and regret guarantees of Algorithm~\ref{alg:BOFUL} under the setting of \emph{returning users} in linear contextual bandits. We first define the setting of returning users that we consider in this section, and then state the performance guarantee for Algorithm~\ref{alg:BOFUL}.

% \xingyu{I now tend to feel that this is kind of misleading in our previous notations and wording. That is we first fix $M_0$ and then tune $B$ (say if $M_0=1$, we choose $B = T$? even contradicts with our previous unique users in some sense).  This is not used in practice. What we used in practice is that we first fix batch size $B$ in advance, and then we chosse how to sample users as decribed in the above example. 
% % Under our assumption of returning users, we have the following guarantee. 
% We are not trying to create batch based on how frequently users contribute. Rather, it is the server to decide how to sample users across different batches.}

% \xingyu{I create the current one in new\_return.tex file and  keep the old one in old\_return.tex unchanged} 

\begin{assumption}[Returning Users]
\label{def:return_def}
For a given time horizon $T \in \Nat$ and batch size $B \in [T]$, any user can participate in \emph{all} $M = T/B$ batches, but within each batch $m \in [M]$, she only contributes once.
\end{assumption}
In addition to the above motivating example, this assumption also captures many practical adaptive learning scenarios such as clinical trials and product recommendations, in which each trial (batch) involves a group of unique people, but the same person may participate in multiple trials~\cite{ren2020batched,schwartz2017customer}.

% \sayak{This does not look like a definition.}\xingyu{I prefer to call it assumption actually.}

% \begin{assumption}[Returning Users]
% \label{ass:return_ass}
% We assume that each user can participate in multiple batches, but within each batch she only contributes once. 
% \end{assumption}
% \sayak{Can we state this inline--not making any assumptions. Just say that each user are now allowed to participate in multiple batches.}\xingyu{I am fine with this:) but we need to emphasize that the user cannot appear twice in the same batch.}
% \sayak{Yes} \xingyu{just go ahead:)}\sayak{I will do this section and exps tomoroo} 
% \xingyu{sure, I will finish the polish for section 3, i.e, the appendix}great \xingyu{I like the current style of section 3.}\sayak{Yes, it looks good. Section 4 is very important for us. Thanks.}\xingyu{while you edit it, you can also have a double check:) haha. I give the intuition for user-level JDP, which you can easily understand. For SDP, it directly follows from composition, no fancy things.}great
% \sayak{Some equation refs are not working I see}
% \xingyu{I will fix them. You just edit your comments. Finally, I will go over to make sure there no warnings of latex.}okay


\begin{theorem}[Performance guarantees (informal)]
\label{thm:return-main}
Under Assumption~\ref{def:return_def}, we obtain the following results for $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$, respectively. 
% \xingyu{we get something like:}
% \begin{align*}
%     R(T) &= dB + \frac{M_0^{1/4}T^{3/4}d^{3/4}}{\epsilon^{1/2} B^{1/4}}\\
%     & = d\frac{T}{M} + d^{3/4}\frac{\sqrt{M_0 T}}{\epsilon^{1/2}} \left(\frac{M}{M_0}\right)^{1/4}
% \end{align*}
% \xingyu{what do you think, Sayak? This one seems not that perfect.}\sayak{for $M_0=1$, we recover Thm 3.2. If $M_0 =M$, we match JDP, Yes, same order. Basically, setting $B=T/M_0$, we match JDP. call?ye}\xingyu{but if $M_0 = 1$, this not true. we cannot set $B$ according to $M_0$. $B$ should not depend on $M_0$. sure zoom} \xingyu{yes. as expected. or $M_0$ same order as $M$, we are fine, right? Not has to be equal, same order is fine? just some constant. Ok, let's use this results?}
% % \xingyu{it seems that this is not clear. In some sense, only in the worst case, it matches central model, i.e., $M_0 = T/B$?}

(i) For any $\epsilon \!\leq\! \frac{2}{B}\log(2/\delta)\sqrt{2T}$ and $\delta \!\in\! (0,1]$, Algorithm~\ref{alg:BOFUL} instantiated using $\cP_{\text{Amp}}$ with noise levels $\sigma_1 \!=\! \sigma_2 \!=\! \frac{16\log(2/\delta)\sqrt{T(\log(5T/\delta))}}{\epsilon{B}}$ is $O(\epsilon,\delta)$-SDP, and enjoys, with high-probability, the regret bound
\begin{align*}
     \text{Reg}(T) = \widetilde{O}\left(\frac{dT}{M} + \sqrt{\frac{MT}{\epsilon}}d^{3/4} \log^{3/4} (T/\delta)\right).
\end{align*}
(ii) For any $\epsilon \!\leq\! 15$, $\delta \!\in\! (0,1/2)$, there exist choices of parameters $g,b \!\in\! \Nat$, $p \!\in\! (0,1/2)$ depending on $B,\epsilon,\delta$ such that Algorithm~\ref{alg:BOFUL} instantiated using $\cP_{\text{Vec}}$ is $(\epsilon,\delta)$-SDP, and, enjoys, with high probability, the regret bound
\begin{align*}
     \text{Reg}(T) \!=\! \widetilde{O}\left(\frac{dT}{M} \!+\!\sqrt{\frac{MT}{\epsilon}}d^{3/4} \log^{3/4} (d^2M/\delta)\right).
\end{align*}

% \begin{align*}
%      \text{Reg}(T) \!=\! \widetilde{O}\left(\frac{dT}{M} \!+\!\frac{\log^{3/4}(d^2M/\delta)}{\epsilon^{1/2}} d^{3/4}\!\sqrt{MT}\right).
% \end{align*}
% Let $B = O(d^{-1/6}\epsilon^{-1/3}T^{2/3}(\log(Td^2/\delta))^{1/2})$, $g = \max\{2\sqrt{B}, d, 4\}$, $p=1/4$ and 
% \begin{align*}
%     b = \frac{ 10^7\cdot \log(2/\delta)\cdot g^2 \cdot T\cdot \left(\log\left(\frac{8\cdot T(d^2+1)}{B\delta}\right)\right)^2}{\epsilon^2B^2}.
% \end{align*}
\end{theorem}
 

% \begin{theorem}[Performance guarantees (informal)]
% \label{thm:return-main}
% % Let Assumption~\ref{ass:bounded} and Assumption~\ref{ass:return_ass} hold. 
% We have the following results for $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$, respectively. 


% (i) Fix any $B \!\in\! \Nat$, $\epsilon \!\leq\! \frac{2}{B}\sqrt{2T\log(2/\delta)}$ and $\delta \!\in\! (0,1]$. Then, Algorithm~\ref{alg:BOFUL} instantiated with $\cP_{\text{Amp}}$ with noise levels $\sigma_1 \!=\! \sigma_2 \!=\! \frac{16\sqrt{T\log(2/\delta)(\log(5T/\delta))}}{\epsilon{B}}$is $O(\epsilon,\delta)$-SDP, and enjoys, with high-probability, the regret bound
% \begin{align*}
%      \text{Reg}(T) = \widetilde{O}\left(dB\log T + \frac{\log^{1/2}(T/\delta)}{\epsilon^{1/2}B^{1/2}} d^{3/4} T\right)~.
% \end{align*}

% (ii) Fix any $B\!\in\! \Nat$, any $\epsilon \!\le\! 15$, and $\delta \!\in\! (0,1/2)$. There exist choices of parameters $g,b \!\in\! \Nat$ and $p \!\in\! (0,1/2)$ depending on $B,\epsilon,\delta$ such that Algorithm~\ref{alg:BOFUL} instantiated with $\cP_{\text{Vec}}$ is $(\epsilon,\delta)$-SDP, and, enjoys, with high probability, the regret
% \begin{align*}
%      \text{Reg}(T) = \widetilde{O}\left(dB\log T +\frac{\log^{3/4}(d^2T/(B\delta))}{\epsilon^{1/2}B^{1/2}} d^{3/4}T\right).
% \end{align*}
% % Let $B = O(d^{-1/6}\epsilon^{-1/3}T^{2/3}(\log(Td^2/\delta))^{1/2})$, $g = \max\{2\sqrt{B}, d, 4\}$, $p=1/4$ and 
% % \begin{align*}
% %     b = \frac{ 10^7\cdot \log(2/\delta)\cdot g^2 \cdot T\cdot \left(\log\left(\frac{8\cdot T(d^2+1)}{B\delta}\right)\right)^2}{\epsilon^2B^2}.
% % \end{align*}
% \end{theorem}


\begin{proof}[Proof sketch]
In contrast to Section~\ref{sec:shuffleModel} for unique users, where $(\epsilon,\delta)$-SDP guarantee for Algorithm~\ref{alg:BOFUL} can be established by showing each batch is $(\epsilon,\delta)$-SDP, we now need to guarantee that outputs of all the batches together have a total privacy loss of $(\epsilon,\delta)$.
This is due to the fact that now each batch can potentially operate on same set of users, and hence, one need to use advanced decomposition to calculate the total privacy loss. This leads to scaling up the noise variance by a multiplicative factor of $O(M)$ at each batch, which eventually leads to the above bound (the additional $M$ factor in $\delta$ also comes from advance composition).
\end{proof}
% \sayak{We need to write here why the noise added is bit high to guarantee privacy. Basically explain a bit where the proof is different from the previous ones. Just to get the reader know that this is achallenging setting.}\xingyu{I think what you have written is already the key:)}
% and the regret in~\eqref{eq:regret_intuition}. That is, we now need to roughly replace $\epsilon$ by $\epsilon/(\sqrt{T/B})$ in~\eqref{eq:regret_intuition}.
% \begin{remark}
% For batch size $B \!=\! O(T^{2/3})$, i.e., when each user is allowed to participate in at most $T^{1/3}$ batches, the regret of Algorithm~\ref{alg:BOFUL} is $\widetilde{O}\left( \frac{T^{2/3}}{\sqrt{\epsilon}}\right)$ for both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$ under the setting of returning users. As before, if $B$ also depends on $\epsilon$, then we can achieve a better regret $\widetilde{O}(T^{2/3}\epsilon^{-1/3})$, see Appendix~\ref{app:return}.
% \end{remark}
% \xingyu{here $B$ needs to be dependent on $\epsilon$, and hence regret is $O(T^{2/3}\epsilon^{-1/3})$ or you just consider $B = T^{2/3}$?}
% \xingyu{We can say a better $\epsilon$ dependence is possible with $B$ depending on $\epsilon$, see Appendix.}\sayak{I consider $B=T^{2/3}$}\xingyu{how about here we also show that when $B$ depends on $\epsilon$, we can have a regret $O(T^2/3\epsilon^{-1/3})$. In the following, we show that central model have the same results for both under same $M$, returning frequency somehow}\sayak{Central model does not have batch concept. People might get confused.}\xingyu{great, I was trying to say the following message: Algorithm 1 matches central model is kind of universal in that for the same different values of $M$, they continue to hold. Not just for $M = T^{1/3}$.}\sayak{I don't think regret will match for every $M$. There is a $dT/M$ term sitting in front.}
%\end{remark}
% Denoting total number of batches $M\!=\!T/B$ in Theorem~\ref{thm:return-main}, we obtain that Algorithm~\ref{alg:BOFUL} achieves regret $\widetilde{O}\left( \sqrt{TM/\epsilon}\right)$ for both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$ under the setting of returning users.
Interestingly, the privacy ($\epsilon,\delta$)-dependent term in above regret bounds match the one that can be achieved in the \emph{user-level} central trust model that handles returning users. Note that, since existing work in the central model of privacy (i.e., under JDP guarantee) assume unique users~\cite{shariff2018differentially}, we first generalize it to handle returning users. This can be viewed as the same form of generalization from \emph{event-level} DP to \emph{user-level} DP under continual observation, where the adjacent relation between two data streams changes from the flip of one single round to the flip of multiple rounds associated with a single user \cite{dwork2010differential}.\footnote{See Appendix~\ref{app:JDP} for formal definitions of event-level and user-level joint differential privacy (JDP).} As in standard notion of DP, one straightforward approach for converting event-level JDP to user-level JDP is to use group privacy~\cite{dwork2014algorithmic}. However, this black-box approach would blow up the terms dependent on $\delta$. To overcome this, we propose a simple modification of original (event-level) algorithm in~\cite{shariff2018differentially} so that it can handle returning users. In particular, user-level JDP can be achieved by scaling up the noise variance by a multiplicative factor of $M_0^2$, if any user participates in at most $M_0$ rounds. This follows from the fact that flipping one user now would change the $\ell_2$ sensitivity of the expanded binary-tree nodes from $O(\sqrt{\log T})$ to $O(M_0\sqrt{\log T})$. Note that we use $M_0$ to distinguish from the number of batches $M$ since there is no batch concept in standard central model. 
This modified version enjoys the following regret guarantee.

% \sayak{State what is the modification in short.}\xingyu{This is just stated in the theorem statement, i.e., reduce $\epsilon$ to $\epsilon/M$.}\sayak{Does that mean noise level is $\frac{M^2\log T}{\epsilon^2}$}\xingyu{yes. basically reduce $\epsilon$ in previous section by a factor of $M$. see the proof sketch below.}


% this modified algorithm attains nearly the same regret bound as in Theorem~\ref{thm:return-main}  under the same value of $B$, i.e., the same number of rounds one user can contribute. 

\begin{proposition}\label{prop:JDP-return}
If any user participates in at most $M_0$ rounds, the algorithm in \cite{shariff2018differentially}, with the above modification to handle user-level privacy, achieves the high-probability regret bound
\begin{align*}
    \text{Reg}(T) = \widetilde{O}\left(d\sqrt{T} + \sqrt{\frac{M_0T}{\epsilon}}d^{3/4} \log^{1/4} (1/\delta) \right).
\end{align*}
\end{proposition}

% with noise variance scaled up by a multiplicative factor of $M^2$ is able to achieve $(\epsilon,\delta)$-JDP (user-level) with a high-probability regret bound 
% \begin{align*}
%     \text{Reg}(T) = \widetilde{O}\left(d\sqrt{T} + \sqrt{\frac{MT}{\epsilon}}d^{3/4} \log^{1/4} (1/\delta) \right).
% \end{align*}

% \begin{proof}[Proof sketch]
% This follows from the fact that flipping one user now would change the $\ell_2$ sensitivity of the expanded binary-tree nodes from $O(\sqrt{\log T})$ to $O(M\sqrt{\log T})$. 
% \end{proof}
% \sayak{Why regret is $d^{3/4}$? ? we should give linear in $d$ term as well.}\xingyu{no, the same as previous CDP. you just check the CDP paper, you can get it. or directly look at our general result. see Lemma 3.9}\sayak{Please make the changes.}\xingyu{which change? in previous sections, you did not write any $d$ term I think.} I changed in the proposition
% \begin{remark}
% Setting $M = T^{1/3}$ yields the regret bound (i.e., $\tilde{O}(d^{5/6}T^{2/3}\epsilon^{-1/3})$) up to logarithmic factor in terms of $1/\delta$ and $T$.
% \end{remark}

\begin{remark}
Comparing Theorem~\ref{thm:return-main} and Proposition~\ref{prop:JDP-return}, we observe that the cost of privacy in the shuffle model is essentially same (upto a log factor) as in the central model under the setting of returning users.
In particular, if $M = M_0=T^{1/3}$ rounds (i.e., the same number of possible returning rounds for any user), the regret is $\widetilde O\left(\frac{T^{2/3}}{\sqrt{\epsilon}}\right)$ in both shuffle and user-level central trust models. 
See Appendix~\ref{app:return} for complete proofs and more details.
% For batch size $B \!=\! O(T^{2/3})$, i.e., when each user is allowed to participate in at most $T^{1/3}$ batches, the regret of Algorithm~\ref{alg:BOFUL} is $\widetilde{O}\left( \frac{T^{2/3}}{\sqrt{\epsilon}}\right)$ for both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$ under the setting of returning users. As before, if $B$ also depends on $\epsilon$, then we can achieve a better regret $\widetilde{O}(T^{2/3}\epsilon^{-1/3})$, see Appendix~\ref{app:return}.
\end{remark}


==> Shuffle Linear Bandit Arxiv/old_return.tex <==
Similar to existing work on differentially private bandits, in previous sections, we have assumed that all participating users are unique, i.e., each user participates in the protocol only at one round. A more practical scenario is that an user can contribute with her data at multiple rounds. For example, consider the mobile medical application described in the introduction. The cloud server can collect one particular user's data during multiple batches to track the effectiveness of its treatment plan over a period, and hence, use same user's data multiple time to update its recommendation algorithm. Motivated by this, we provide privacy and regret guarantees of Algorithm~\ref{alg:BOFUL} under the setting of \emph{returning users} in linear contextual bandits. We first define the setting of returning users that we consider in this section, and then state the performance guarantee for Algorithm~\ref{alg:BOFUL}.
\begin{definition}[Returning users (informal)]
\label{def:return_def}
Each user can participate in multiple batches, but within each batch she only contributes once. 
\end{definition}


% \begin{assumption}[Returning Users]
% \label{ass:return_ass}
% We assume that each user can participate in multiple batches, but within each batch she only contributes once. 
% \end{assumption}
% \sayak{Can we state this inline--not making any assumptions. Just say that each user are now allowed to participate in multiple batches.}\xingyu{I am fine with this:) but we need to emphasize that the user cannot appear twice in the same batch.}
% \sayak{Yes} \xingyu{just go ahead:)}\sayak{I will do this section and exps tomoroo} 
% \xingyu{sure, I will finish the polish for section 3, i.e, the appendix}great \xingyu{I like the current style of section 3.}\sayak{Yes, it looks good. Section 4 is very important for us. Thanks.}\xingyu{while you edit it, you can also have a double check:) haha. I give the intuition for user-level JDP, which you can easily understand. For SDP, it directly follows from composition, no fancy things.}great
% \sayak{Some equation refs are not working I see}
% \xingyu{I will fix them. You just edit your comments. Finally, I will go over to make sure there no warnings of latex.}okay


\begin{theorem}[Performance guarantees (informal)]
\label{thm:return-main}
If any user participates in at most $M_0$ rounds (i.e., $M_0$ batches by above definition), then running Algorithm~\ref{alg:BOFUL} with batchsize $B=T/M_0$, we obtain the following results for $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$, respectively. 
\xingyu{I now tend to feel that this is kind of misleading. That is we first fix $M_0$ and then tune $B$. But if $M_0=1$, we choose $B = T$?. This is not used in practice. What we used in practice is that we first fix batch size $B$ in advance, and then we chosse how to sample users. Under our assumption of returning users, we have the following guarantee. We are not trying to create batch based on how frequently users contribute. Rather, it is the server to decide how to sample users across different batches.}

(i) For any $\epsilon \!\leq\! \frac{2}{B}\sqrt{2T\log(2/\delta)}$ and $\delta \!\in\! (0,1]$, $\cP_{\text{Amp}}$ with noise levels $\sigma_1 \!=\! \sigma_2 \!=\! \frac{16\sqrt{T\log(2/\delta)(\log(5T/\delta))}}{\epsilon{B}}$ is $O(\epsilon,\delta)$-SDP, and enjoys, with high-probability, the regret bound
\begin{align*}
     \text{Reg}(T) = \widetilde{O}\left(\frac{dT}{M_0}\log T + \frac{\log^{1/2}(T/\delta)}{\epsilon^{1/2}} d^{3/4} \sqrt{M_0T}\right).
\end{align*}
(ii) For any $\epsilon \!\leq\! 15$, $\delta \!\in\! (0,1/2)$, there exist choices of parameters $g,b \!\in\! \Nat$, $p \!\in\! (0,1/2)$ depending on $B,\epsilon,\delta$ such that $\cP_{\text{Vec}}$ is $(\epsilon,\delta)$-SDP, and, enjoys the regret bound
\begin{align*}
     \text{Reg}(T) \!=\! \widetilde{O}\left(\frac{dT}{M_0}\log T \!+\!\frac{\log^{3/4}(d^2M_0/\delta)}{\epsilon^{1/2}} d^{3/4}\!\sqrt{M_0T}\right).
\end{align*}
% Let $B = O(d^{-1/6}\epsilon^{-1/3}T^{2/3}(\log(Td^2/\delta))^{1/2})$, $g = \max\{2\sqrt{B}, d, 4\}$, $p=1/4$ and 
% \begin{align*}
%     b = \frac{ 10^7\cdot \log(2/\delta)\cdot g^2 \cdot T\cdot \left(\log\left(\frac{8\cdot T(d^2+1)}{B\delta}\right)\right)^2}{\epsilon^2B^2}.
% \end{align*}
\end{theorem}
 

% \begin{theorem}[Performance guarantees (informal)]
% \label{thm:return-main}
% % Let Assumption~\ref{ass:bounded} and Assumption~\ref{ass:return_ass} hold. 
% We have the following results for $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$, respectively. 


% (i) Fix any $B \!\in\! \Nat$, $\epsilon \!\leq\! \frac{2}{B}\sqrt{2T\log(2/\delta)}$ and $\delta \!\in\! (0,1]$. Then, Algorithm~\ref{alg:BOFUL} instantiated with $\cP_{\text{Amp}}$ with noise levels $\sigma_1 \!=\! \sigma_2 \!=\! \frac{16\sqrt{T\log(2/\delta)(\log(5T/\delta))}}{\epsilon{B}}$is $O(\epsilon,\delta)$-SDP, and enjoys, with high-probability, the regret bound
% \begin{align*}
%      \text{Reg}(T) = \widetilde{O}\left(dB\log T + \frac{\log^{1/2}(T/\delta)}{\epsilon^{1/2}B^{1/2}} d^{3/4} T\right)~.
% \end{align*}

% (ii) Fix any $B\!\in\! \Nat$, any $\epsilon \!\le\! 15$, and $\delta \!\in\! (0,1/2)$. There exist choices of parameters $g,b \!\in\! \Nat$ and $p \!\in\! (0,1/2)$ depending on $B,\epsilon,\delta$ such that Algorithm~\ref{alg:BOFUL} instantiated with $\cP_{\text{Vec}}$ is $(\epsilon,\delta)$-SDP, and, enjoys, with high probability, the regret
% \begin{align*}
%      \text{Reg}(T) = \widetilde{O}\left(dB\log T +\frac{\log^{3/4}(d^2T/(B\delta))}{\epsilon^{1/2}B^{1/2}} d^{3/4}T\right).
% \end{align*}
% % Let $B = O(d^{-1/6}\epsilon^{-1/3}T^{2/3}(\log(Td^2/\delta))^{1/2})$, $g = \max\{2\sqrt{B}, d, 4\}$, $p=1/4$ and 
% % \begin{align*}
% %     b = \frac{ 10^7\cdot \log(2/\delta)\cdot g^2 \cdot T\cdot \left(\log\left(\frac{8\cdot T(d^2+1)}{B\delta}\right)\right)^2}{\epsilon^2B^2}.
% % \end{align*}
% \end{theorem}


\begin{proof}[Proof sketch]
In contrast to Section~\ref{sec:shuffleModel}, where $(\epsilon,\delta)$-SDP can guaranteed for Algorithm~\ref{alg:BOFUL} by showing each batch is $(\epsilon,\delta)$-SDP, we now need to guarantee that outputs of all the batches together have a total privacy loss of $(\epsilon,\delta)$.
This is due to the fact that now each batch can potentially operate on same set of users, and hence, one need to resort to advanced decomposition theorem. This requires scaling up the noise variance by a multiplicative factor of $O(M_0)$ at each batch, which eventually leads to the above regret bound.
\end{proof}
% \sayak{We need to write here why the noise added is bit high to guarantee privacy. Basically explain a bit where the proof is different from the previous ones. Just to get the reader know that this is achallenging setting.}\xingyu{I think what you have written is already the key:)}
% and the regret in~\eqref{eq:regret_intuition}. That is, we now need to roughly replace $\epsilon$ by $\epsilon/(\sqrt{T/B})$ in~\eqref{eq:regret_intuition}.
% \begin{remark}
% For batch size $B \!=\! O(T^{2/3})$, i.e., when each user is allowed to participate in at most $T^{1/3}$ batches, the regret of Algorithm~\ref{alg:BOFUL} is $\widetilde{O}\left( \frac{T^{2/3}}{\sqrt{\epsilon}}\right)$ for both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$ under the setting of returning users. As before, if $B$ also depends on $\epsilon$, then we can achieve a better regret $\widetilde{O}(T^{2/3}\epsilon^{-1/3})$, see Appendix~\ref{app:return}.
% \end{remark}
% \xingyu{here $B$ needs to be dependent on $\epsilon$, and hence regret is $O(T^{2/3}\epsilon^{-1/3})$ or you just consider $B = T^{2/3}$?}
% \xingyu{We can say a better $\epsilon$ dependence is possible with $B$ depending on $\epsilon$, see Appendix.}\sayak{I consider $B=T^{2/3}$}\xingyu{how about here we also show that when $B$ depends on $\epsilon$, we can have a regret $O(T^2/3\epsilon^{-1/3})$. In the following, we show that central model have the same results for both under same $M$, returning frequency somehow}\sayak{Central model does not have batch concept. People might get confused.}\xingyu{great, I was trying to say the following message: Algorithm 1 matches central model is kind of universal in that for the same different values of $M$, they continue to hold. Not just for $M = T^{1/3}$.}\sayak{I don't think regret will match for every $M$. There is a $dT/M$ term sitting in front.}
%\end{remark}
% Denoting total number of batches $M\!=\!T/B$ in Theorem~\ref{thm:return-main}, we obtain that Algorithm~\ref{alg:BOFUL} achieves regret $\widetilde{O}\left( \sqrt{TM/\epsilon}\right)$ for both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$ under the setting of returning users.
Interestingly, the privacy ($\epsilon,\delta$) dependent term in above regret bounds match the one that can be achieved in the central trust model (under the setting of returning users). Since existing work in the central model of privacy (i.e., under JDP guarantee) assume unique users~\cite{shariff2018differentially}, we first generalize it to handle returning users. This generalization can be viewed as the same as from event-level DP to user-level DP under continual observation in~\cite{dwork2010differential}, where the adjacent relation between two data streams changes from the flip of one single round to the flip of multiple rounds associated with a single user.\footnote{See Appendix~\ref{app:JDP} for formal definitions of event-level and user-level joint differential privacy (JDP).} As in standard notion of DP, one straightforward approach for converting event-level JDP to user-level JDP is to use group privacy~\cite{dwork2014algorithmic}. However, this black-box approach would blow up the terms dependent on $\delta$. To overcome this, we propose a simple modification of original (event-level) algorithm in~\citet{shariff2018differentially} so that it can handle returning users. In particular, user-level JDP can be achieved by scaling up the noise variance by a multiplicative factor of $M_0^2$, if any user participates in at most $M_0$ rounds. This follows from the fact that flipping one user now would change the $\ell_2$ sensitivity of the expanded binary-tree nodes from $O(\sqrt{\log T})$ to $O(M\sqrt{\log T})$.
This modified version enjoys the following regret guarantee.

% \sayak{State what is the modification in short.}\xingyu{This is just stated in the theorem statement, i.e., reduce $\epsilon$ to $\epsilon/M$.}\sayak{Does that mean noise level is $\frac{M^2\log T}{\epsilon^2}$}\xingyu{yes. basically reduce $\epsilon$ in previous section by a factor of $M$. see the proof sketch below.}


% this modified algorithm attains nearly the same regret bound as in Theorem~\ref{thm:return-main}  under the same value of $B$, i.e., the same number of rounds one user can contribute. 

\begin{proposition}\label{prop:JDP-return}
If any user participates in at most $M_0$ rounds, the algorithm in~\citet{shariff2018differentially}, with the above modification to handle user-level privacy, achieves the high-probability regret bound
\begin{align*}
    \text{Reg}(T) = \widetilde{O}\left(d\sqrt{T} + \sqrt{\frac{M_0T}{\epsilon}}d^{3/4} \log^{1/4} (1/\delta) \right).
\end{align*}
\end{proposition}
% with noise variance scaled up by a multiplicative factor of $M^2$ is able to achieve $(\epsilon,\delta)$-JDP (user-level) with a high-probability regret bound 
% \begin{align*}
%     \text{Reg}(T) = \widetilde{O}\left(d\sqrt{T} + \sqrt{\frac{MT}{\epsilon}}d^{3/4} \log^{1/4} (1/\delta) \right).
% \end{align*}

% \begin{proof}[Proof sketch]
% This follows from the fact that flipping one user now would change the $\ell_2$ sensitivity of the expanded binary-tree nodes from $O(\sqrt{\log T})$ to $O(M\sqrt{\log T})$. 
% \end{proof}
% \sayak{Why regret is $d^{3/4}$? ? we should give linear in $d$ term as well.}\xingyu{no, the same as previous CDP. you just check the CDP paper, you can get it. or directly look at our general result. see Lemma 3.9}\sayak{Please make the changes.}\xingyu{which change? in previous sections, you did not write any $d$ term I think.} I changed in the proposition
% \begin{remark}
% Setting $M = T^{1/3}$ yields the regret bound (i.e., $\tilde{O}(d^{5/6}T^{2/3}\epsilon^{-1/3})$) up to logarithmic factor in terms of $1/\delta$ and $T$.
% \end{remark}

\begin{remark}
Comparing Theorem~\ref{thm:return-main} and Proposition~\ref{prop:JDP-return}, we observe that the cost of privacy in the shuffle model is essentially same (upto a log factor) as in the central model under the setting of returning users.
In particular, if users participate in at most $M_0=T^{1/3}$ round, the regret is $\widetilde O\left(\frac{T^{2/3}}{\sqrt{\epsilon}}\right)$ in both shuffle and central trust models.
% For batch size $B \!=\! O(T^{2/3})$, i.e., when each user is allowed to participate in at most $T^{1/3}$ batches, the regret of Algorithm~\ref{alg:BOFUL} is $\widetilde{O}\left( \frac{T^{2/3}}{\sqrt{\epsilon}}\right)$ for both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$ under the setting of returning users. As before, if $B$ also depends on $\epsilon$, then we can achieve a better regret $\widetilde{O}(T^{2/3}\epsilon^{-1/3})$, see Appendix~\ref{app:return}.
\end{remark}


==> Shuffle Linear Bandit Arxiv/practical.tex <==
\section{Simulation Results}




\begin{figure}[t]\centering
\begin{subfigure}[t]{.3\linewidth}
		\centering
			\includegraphics[width = 2.1in]{Figures/new_eps_1_by_2.pdf}
			\caption{$\epsilon = 0.2$}
		\end{subfigure} \ \
		\begin{subfigure}[t]{.3\linewidth}
		\centering
			\includegraphics[width = 2.1in]{Figures/new_eps_1.pdf}
			\caption{$\epsilon = 1$}
		\end{subfigure} \ \
		\begin{subfigure}[t]{.3\linewidth}
		\centering
			\includegraphics[width = 2.1in]{Figures/new_eps_10.pdf}
			\caption{$\epsilon = 10$}
		\end{subfigure}
		 \vspace{-1mm}
		\caption{\footnotesize{Comparison of cumulative regret for LinUCB (non-private), LinUCB-JDP (central model), LinUCB-SDP (shuffle model) and LinUCB-LDP (local model) with varying privacy level $\epsilon=0.2$ (a), $\epsilon=1$ (b) and $\epsilon=10$ (c). For $\epsilon=0.2$ (higher privacy level), gap between private and non-private regret is higher as compared to $\epsilon=10$ (lower privacy level). In all cases, regret of LinUCB-SDP lies perfectly in between LinUCB-JDP and LinUCB-LDP, achieving finer regret-privacy trade-off.}  }\label{fig:all_algos}
		\vspace{0mm}
\end{figure}


In this section, we empirically evaluate the regret performance of Algorithm~\ref{alg:BOFUL} (under shuffle model), which we abbreviate as LinUCB-SDP-Amp and LinUCB-SDP-Vec when instantiated with $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$, respectively. We compare them with the algorithms of \cite{shariff2018differentially} and \cite{zheng2020locally} under central and local models, which we call LinUCB-JDP and LinUCB-LDP, respectively. We benchmark these against the non-private algorithm of \cite{abbasi2011improved}, henceforth referred as LinUCB. For all the experiments, we consider $100$ arms, set $T = 20000$ rounds, and average our results
over 50 randomly generated bandit instances. Each instance is characterized by an
(unknown) parameter $\theta^*$ and feature vectors of dimension $d=5$. To ensure boundedness, similar to~\cite{vaswani2020old}, 
we generate each $\theta^*$ and feature vectors by sampling a $(d\!-\!1)$-dimensional vectors of norm $1/\sqrt{2}$ uniformly at random, and append it with a $1/\sqrt{2}$ entry. We consider Bernoulli $\lbrace 0,1\rbrace$ rewards.
We fix $\delta\!=\!0.1$ and plot the results for varying privacy level $\epsilon \in \lbrace 0.2,1,10\rbrace$ in Figure~\ref{fig:all_algos}. We use Batchsize $B=20$ for LinUCB-SDP. We postpone the results for $d=10,15$ to Appendix~\ref{app:sim}.
% \footnote{We stick to $\cP_{\text{Amp}}$ as implementing the encoding scheme in $\cP_{\text{Vec}}$ requires further care. However, one can always simulate the noise added by $\cP_{\text{Vec}}$ during each batch, and study its effect on the regret.}
% \xingyu{I may try to implement this before the ddl and you can plug it into your code to see the difference. }
% \sayak{It might take a lot of time.}
% \xingyu{I will control the time. if it costs me too much, I will stop it.}\sayak{I think we are fine with amp at this point. Anyway, if you have time, please.}\xingyu{sure, just a try:)}\sayak{Write a class as LinUCB}



% \begin{figure*}[t]\centering
% 		\begin{subfigure}{2in}
% 			\includegraphics[width = 1.65in]{Figures/Bernoulli (d=5,eps=0.2,delta=0.1,B=20).pdf}
% 			\caption{1 }
% 		\end{subfigure}\ \
% 		\begin{subfigure}{2in}
% 			\includegraphics[width = 1.65in]{Figures/Bernoulli (d=5,eps=1,delta=0.1,B=20).pdf}
% 			\caption{2}
% 		\end{subfigure}\ \
% 		\begin{subfigure}{2in}
% 			\includegraphics[width = 1.65in]{Figures/Bernoulli (d=5,eps=10,delta=0.1,B=20).pdf}
% 			\caption{3}
% 		\end{subfigure}
% 		 \vspace{0mm}
% 		\caption{figure }\label{fig:regret}
% 		\vspace{0mm}
% \end{figure*}


% \begin{figure*}[h]\centering
%     \begin{subfigure}[b]{0.32\textwidth}
%     \includegraphics[scale=0.25]{Figures/Bernoulli (d=5,eps=0.2,delta=0.1,B=20).pdf}
%     \caption{$\epsilon = 0.2$}
%     \end{subfigure}\ \
%     \begin{subfigure}[b]{0.32\textwidth}
%     \includegraphics[scale=0.25]{Figures/Bernoulli (d=5,eps=1,delta=0.1,B=20).pdf}
%     \caption{$\epsilon = 1$}
%     \end{subfigure}\ \
%     \begin{subfigure}[b]{0.32\textwidth}
%     \includegraphics[scale=0.25]{Figures/Bernoulli (d=5,eps=10,delta=0.1,B=20).pdf}
%     \caption{$\epsilon = 10$}
%     \end{subfigure}\\
%     % \begin{subfigure}[b]{0.32\textwidth}
%     % \includegraphics[scale=0.25]{syn_student.eps}
%     % \caption{Non-private, Synthetic data, $k_{\text{SE} }$}
%     % \end{subfigure}\ \
%     % \begin{subfigure}[b]{0.32\textwidth}
%     % \includegraphics[scale=0.25]{light.eps}
%     % \caption{Non-private, Light sensor data}
%     % \end{subfigure}\ \
%     % \begin{subfigure}[b]{0.32\textwidth}
%     % \includegraphics[scale=0.25]{fin.eps}
%     % \caption{Non-private, Stock market data}
%     % \end{subfigure}
% \caption{figure}\label{fig:regret}
% \end{figure*}


% \begin{figure}[H]
% 	\centering
% 	\vskip 0mm
% 	\includegraphics[width=0.8\linewidth,height=0.5\linewidth]{Figures/Bernoulli (d=5,eps=0.2,delta=0.1,B=20).pdf}
% 	\vskip -1mm
%  	\includegraphics[width=0.8\linewidth,height=0.5\linewidth]{Figures/Bernoulli (d=5,eps=1,delta=0.1,B=20).pdf}
%  	\vskip -1mm
%  	\includegraphics[width=0.8\linewidth,height=0.5\linewidth]{Figures/Bernoulli (d=5,eps=10,delta=0.1,B=20).pdf}
%  	\vskip -5mm
% \caption{\footnotesize{ Comparison of cumulative regret for LinUCB (non-private), LinUCB-JDP (central model), LinUCB-SDP (shuffle model) and LinUCB-LDP (local model) with varying privacy level $\epsilon=0.2$ (top), $\epsilon=1$ (middle) and $\epsilon=10$ (bottom). For $\epsilon=0.2$ (higher privacy level), gap between private and non-private regret is higher as compared $\epsilon=10$ (lower privacy level). In all cases, regret of LinUCB-SDP lies perfectly in between LinUCB-JDP and LinUCB-LDP, achieving finer regret-privacy trade-off.\xingyu{for $\epsilon = 10$, it does not satisfy the condition $\epsilon \le 1/\sqrt{B}$ required by Pamp. This is another motivation for us to plot Pvec mechanism. This will significantly showcase our results. Another simple plot could be replace existing noise in SDP and JDP by the one in the returning users, and we can see the regret will be close. I think this modification is simple, basically scale the noise. }\sayak{I observe that $Pvec $ similar perfromance like $Pamp$. Let's plot both?}\xingyu{Wow!! Great, definitely:) Thanks Sayak} \xingyu{please see the following page on placing these figures across columns}\sayak{Thanks. Should we put both shuffle protocol together with others?} \xingyu{Yes, that would be great. That is, in the first two figures $\epsilon = 0.2, 1$, we add the curve for Pvec. And for the last one $\epsilon = 10$, we only plot Pvec since Pamp does not satisfy the condition. Then, we can do the same thing for the returning users case by simply scaling the noise. Thus, in total we have $6$ figures in the main content.  }\sayak{Then, we won't have LDP. But, this will be just simulating the noise. Right? Not entirely the practical scenario. Anyway what will be the extra noise compared to single user?} \xingyu{Yes, LDP for user-level is tricky. That's the reason we did not want to consider it. We just compare SDP vs JDP in the case of returning users (i.e., user-level). The modified noise is given by the proof sketch of Theorem 4.2 and the Proposition 4.3. Yes, kind of simulating noise. But, I think it is totally fine. }\sayak{I am doing B=20. Pamp can by plotted only epsilon= 0.2 or lower. I think we can plot Pamp for all. The result was just theory. \xingyu{Now, $\epsilon$ for Pamp needs to be less than $\sqrt{\frac{\log(2/\delta)}{B}}$, slightly larger. Yes. we can plot. Or we just plot $\epsilon = 0.2$ for Pamp and for larger $\epsilon$, we plot Pvec.}\sayak{Okay.}}
% }}
% \vskip -3mm
% \label{fig:all_algos}
% \end{figure}
From Figure~\ref{fig:all_algos}, we observe that the regret performance of LinUCB-SDP (under both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$) is indeed better than LinUCB-LDP. In addition, it is not surprising that LinUCB-SDP incurs a larger regret than
LinUCB-JDP. Moreover, the regret performance of LinUCB-SDP (in fact for any private algorithm) comes closer to that of LinUCB as $\epsilon$ increases, i.e, as the privacy guarantee becomes weaker. The experimental findings are
consistent with our theoretical results.

%  Our results are also greatly impacted by the batchsize $B$, as Figure ... suggests.

% \xingyu{I am just wondering the performance comparsion between $\cP_{amp}$ and $\cP_{vec}$?}
% \sayak{Have not done it. Will try to do. Anyway, for practice, it doesn't add much value since can't be implemented. Will try simulate and put it in appendix.}

% \begin{remark}
% The above shuffle-model LCB naturally reduces to the standard sequential learning model when $B=1$ since the shuffler now is simply an identity mapping. Thus, it is not only for SDP, but can be used to recover previous private LCB algorithms under JDP and LDP. Thus, to some extent, a LCB protocol given by $\cP = (\cR, \cS, \cA)$ offers us a generic view of LCB under different trust models, which will be explored later.
% \end{remark}

% \begin{remark}
% The above SDP is equivalent to one-round SDP for each batch when all the $T$ users are unique, which is assumed for the main body of this paper. This equivalence holds by parallel-composition of DP on disjoint datasets. However, when some users participate in multiple batches, the two notions are not equivalent anymore. In this case, to guarantee $(\epsilon,\delta)$-SDP, one needs to resort to advanced (sequential) composition of DP to bound the total privacy loss across all possible $M$ outputs. This will be formally addressed in Section [].
% \end{remark}

% \sayak{Will put these remarks after results are written.}


% \subsection{Returning Users}
% As the same with existing works on differentially private bandits, in the previous sections, we assume that all participating users are unique, i.e., each user only participates at one time step. However, a more practical scenario is that one user can contribute at multiple rounds. Take our mobile medical application for example, the cloud server can collect one particular user's data during multiple batches to track the effectiveness of its treatment plan over a period. Unlike the previous sections where $(\epsilon,\delta)$-SDP follows from $(\epsilon,\delta)$-SDP for each batch, we now need to guarantee that all the $M$ outputs have a total privacy loss of $(\epsilon,\delta)$. 

% We first explicitly define the setting of returning users in our paper.

% \begin{assumption}[Returning Users]
% \label{ass:return_ass}
% We assume that each user can participate in multiple batches, but within each batch she only contributes once. 
% \end{assumption}

% Then, we have the following theorem. 

% \begin{theorem}[SDP under returning users]
% \label{thm:return-main}
% Let Assumption~\ref{ass:bounded} and Assumption~\ref{ass:return_ass} hold. Then, we have the following results for $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$, respectively. 


% (i) For any $\epsilon \in [0,\frac{2}{B}\sqrt{2T\log(2/\delta)}]$, $\delta \in (0,1]$ and $B = O(d^{-1/6}\epsilon^{-1/3}T^{2/3}(\log(T/\delta))^{1/3})$, let $\sigma_1 = \sigma_2 = \frac{16\sqrt{T\log(2/\delta)(\log(5T/\delta))}}{\epsilon{B}}$. Then, $\cP_{\text{Amp}}$ is $O(\epsilon,\delta)$-SDP with regret 
% \begin{align*}
%      R(T) = \tilde{O}\left(d^{5/6} T^{2/3}\epsilon^{-1/3}\left(\log(T/\delta)\right)^{1/3}\right).
% \end{align*}

% (ii) For any $\epsilon \le 15$, $\delta \in (0,1/2)$. Let $B = O(d^{-1/6}\epsilon^{-1/3}T^{2/3}(\log(Td^2/\delta))^{1/2})$, $g = \max\{2\sqrt{B}, d, 4\}$, $p=1/4$ and 
% \begin{align*}
%     b = \frac{ 10^7\cdot \log(2/\delta)\cdot g^2 \cdot T\cdot \left(\log\left(\frac{8\cdot T(d^2+1)}{B\delta}\right)\right)^2}{\epsilon^2B^2}.
% \end{align*}
% Then, $\cP_{\text{Vec}}$ is $(\epsilon,\delta)$-SDP with regret 
% \begin{align*}
%       R(T) = \tilde{O}\left(d^{5/6} T^{2/3}\epsilon^{-1/3}\left(\log(d^2T/\delta)\right)^{1/2}\right).
% \end{align*}
% \end{theorem}
% \begin{proof}[Proof sketch]
% This high-level idea follows from advanced composition theorem and the regret in~\eqref{eq:regret_intuition}. That is, we now need to roughly replace $\epsilon$ by $\epsilon/(\sqrt{T/B})$ in~\eqref{eq:regret_intuition}.
% \end{proof}

% Interestingly, the above regret bound matches the one in the central model under the setting of returning users. Note that since existing work in the central model (i.e., JDP) assumes unique users, we first generalize it to handle returning users (see Definition~\ref{def:JDP-user} in Appendix). This generalization can be viewed as the same as from event-level DP to user-level DP under continual observation in~\cite{dwork2010differential}, where the adjacent relation between two data streams changes from the flip of one single round to the flip of multiple rounds associated with a single user.  As in standard DP, one straightforward approach to convert event-level DP to user-level DP is to use group privacy~\cite{dwork2014algorithmic}. However, this black-box approach will blow up the term related to $\delta$. To overcome this, we propose a simple modification of original event-level algorithm in~\cite{shariff2018differentially} with a proper scaling of the noise. In particular, this modified algorithm attains nearly the same regret bound as in Theorem~\ref{thm:return-main}  under the same value of $B$, i.e., the same number of rounds one user can contribute. 

% \begin{theorem}
% Let Assumption~\ref{ass:bounded} hold. If any user appears at most $M$ rounds, the algorithm in~\cite{shariff2018differentially} with private budget $\epsilon$ scaled down to $\epsilon/M$ is able to achieve $(\epsilon,\delta)$-JDP (user-level) with a high-probability regret bound 
% \begin{align*}
%     R(T) = \widetilde{O}\left(d^{3/4} \sqrt{MT} \frac{(\log(1/\delta))^{1/4}}{\sqrt{\epsilon}}  \right).
% \end{align*}
% \end{theorem}
% \begin{proof}[Proof sketch]
% This follows from the fact that flipping one user now would change the $l_2$ sensitivity of the expanded binary-tree nodes from $O(\sqrt{\log T})$ to $O(M\sqrt{\log T})$. 
% \end{proof}
% \begin{remark}
% Setting $M = T/B$ where $B$ in Theorem~\ref{thm:return-main} yields the same regret bound (i.e., $\tilde{O}(d^{5/6}T^{2/3}\epsilon^{-1/3})$) up to logarithmic factor in terms of $1/\delta$ and $T$.
% \end{remark}

% % To the best of our knowledge, almost all existing works on differential private bandits assume that users are unique, i.e., each user only participates once in the learning process. However, in practice, 


% % \paragraph{Returning users}
% % \xingyu{Another key question in this section is whether we should change LDP definition since one user can now send data at multiple rounds. We can choose to keep the current one as everytime $\epsilon$-LDP or we need to define the overall privacy loss of a user over $M$ rounds is $\epsilon$ like SDP. Then, we have to use advanced composition also for LDP.  }\xingyu{Another option is that in this section, we only talk about SDP/JDP and their matching regrets, which will avoid further confusion but still delivery the main message. }
% % \sayak{Let's not change the definitions at this point. Just tell it in words. We can focus on matching JDP regret in this section.}

\section{Concluding Remarks}
\label{sec:conclude}
We conclude by discussing some important theoretical and practical aspects about shuffle protocols, and in general, about privacy in linear contextual bandits.

\textbf{Communications.}
In the protocol $\cP_{\text{Amp}}$, each participating user at each round need to send one $d$-dimensional real vector and one $d\times d$ real matrix.  On the other hand, the protocol $\cP_{\text{Vec}}$ only communicates $0/1$ bits. In particular, each participating user at each round sends out a total of $O(d^2(g+b))$ bits, where $g+b \approx \sqrt{B} + \log(1/\delta)/\epsilon^2$. Hence, $\cP_{\text{Vec}}$ might be more feasible in practice than $\cP_{\text{Amp}}$.



\textbf{Batched algorithms for local and central models.} Existing work on differentially private linear contextual bandits under both local and central models perform sequential update, i.e., the model estimates are updated after each round. As mentioned before, this may not be feasible in practice due to computational load. Fortunately, our proposed algorithm (Algorithm~\ref{alg:BOFUL}) along with its generic regret bound (Lemma~\ref{lem:subG-main}) also offers a simple way to design and analyze private algorithms for local and central models with batched update. In particular, we show that it suffices to update after every $B=\widetilde{O}(T^{3/4})$ rounds to achieve the same privacy-regret trade-off as in the sequential local model and every $B=\widetilde{O}(\sqrt{T})$ to match the sequential central model. See Appendix~\ref{sec:batched} for the details.

% To start with, for the batched algorithm in the local model, one can simply replace the shuffler in Algorithm~\ref{alg:BOFUL} by an identity mapping while using the same local randomizer as in~\cite{zheng2020locally} (i.e., Gaussian mechanism). We call this algorithm $\emph{Batched-Local-LinUCB}$. Thanks to Theorem~\ref{cor:subG-main}, we have the following privacy and regret guarantees. 
% \begin{theorem}
% Let Assumption~\ref{ass:bounded} hold. Fix any $\epsilon_0 \in [0,1]$, $\delta_0 \in (0,1]$ and $\alpha \in [0,1]$, let $\sigma_1 = \sigma_2 = \frac{4\sqrt{2\log(2.5/\delta_0)}}{\epsilon_0}$. Then, for all $B \in [T]$, Bathed-Local-LinUCB is $(\epsilon_0,\delta_0)$-LDP and with probability at least $1-2\alpha$
% \begin{align*}
%     R(T) = \tilde{O}\left(dB + T^{3/4}d^{3/4}\frac{(\log(1/\delta))^{1/4}}{\sqrt{\epsilon}}\log(T/\alpha)\right).
% \end{align*}
% \end{theorem}

% \begin{remark}
% The above theorem indicates that it suffices to update every $B = \tilde{O}(T^{3/4})$ to ensure the same privacy and regret guarantees as in the sequential case.
% \end{remark}

% For the batched algorithm in the central model, we can make the following simple modification over the sequential one in~\cite{shariff2018differentially}, which relies on the seminal tree-based algorithm~\cite{chan2010private} at the central server (analyzer) to balance between privacy and regret. In the batched case, instead of updating the binary-tree nodes after every round, the server updates them only after each batch by treating the the sum of the statistics (i.e., vectors or matrices) within the batch as a single new observation. We call this algorithm \emph{Batched-Central-LinUCB}.
% With this modification and Theorem~\ref{ass:subG-main}, we have the following privacy and regret guarantees. 
% % That is, the binary-tree now only has $M$ leaf nodes and each internal node 
% \begin{theorem}
% Let Assumption~\ref{ass:bounded} hold. Fix any $\epsilon \in [0,1]$, $\delta \in (0,1]$ and $\alpha \in [0,1]$. Then, for all $B \in [T]$, Bathed-Central-LinUCB is $(\epsilon,\delta)$-JDP and with probability at least $1-2\alpha$
% \begin{align*}
%     R(T) = \tilde{O}\left(dB + \sqrt{T}d^{3/4}\frac{(\log(1/\delta))^{1/4}}{\sqrt{\epsilon}}\log(T/\alpha)\right).
% \end{align*}
% \end{theorem}
% \begin{remark}
% The above theorem indicates that it suffices to update every $B = \tilde{O}(\sqrt{T})$ to attain the same privacy-regret trade-off as in the sequential case.
% \end{remark}



\textbf{Adaptive model update.}
One might wonder whether we can further reduce the update frequency to $O(\log T)$ via an adaptive model update schedule based on the standard determinant trick (Lemma 12 of~\cite{abbasi2011improved}). In this approach, the key step is to establish that $\norm{\phi(c,a)}_{V_{\tau_t}^{-1}} \!\leq\! \eta \norm{\phi(c,a)}_{V_{t}^{-1}}$, where $\tau_t \!<\! t$ is the most recent model update time before $t$. To this end, if one uses the determinant trick, one can obtain that
\begin{align*}
    \norm{\phi(c,a)}_{V_{\tau_t}^{-1}} \leq \sqrt{\frac{\det(V_t)}{\det(V_{\tau_t})}} \norm{\phi(c,a)}_{V_{t}^{-1}},
\end{align*}
\emph{if the condition $V_t \succeq V_{\tau_t}$ holds}. Note that this is true in the non-private setting. However, this does not necessarily hold in private settings due to the added noise, which, to the best of our knowledge, is the key analytical gap in the current proof of the main result (Theorem 10) in~\cite{garcelon2021privacy}. As we can see, this issue exists in all three trust models when one needs to use the \emph{noisy} design matrix to determine the update frequency via the determinant trick.


\textbf{Future work.}
One immediate future research direction is to address the above adaptive model update in the private settings. 
We also believe our framework can be generalized to design shuffle private algorithms for reinforcement learning with linear function approximation (e.g., linear mixture Markov decision processes (MDPs)) to 
achieve finer trade-off compared to the local model~\cite{liao2021locally} and the central model~\cite{zhou2022differentially}.

% \xingyu{we can add more here if space permits. I just want to make two columns to align:) i.e., use up all the space.}\sayak{Yes, we can. I might make some writing changes tomorrow.}\xingyu{great! I make some comments in the main part as well.}





==> old_return.tex <==
Similar to existing work on differentially private bandits, in previous sections, we have assumed that all participating users are unique, i.e., each user participates in the protocol only at one round. A more practical scenario is that an user can contribute with her data at multiple rounds. For example, consider the mobile medical application described in the introduction. The cloud server can collect one particular user's data during multiple batches to track the effectiveness of its treatment plan over a period, and hence, use same user's data multiple time to update its recommendation algorithm. Motivated by this, we provide privacy and regret guarantees of Algorithm~\ref{alg:BOFUL} under the setting of \emph{returning users} in linear contextual bandits. We first define the setting of returning users that we consider in this section, and then state the performance guarantee for Algorithm~\ref{alg:BOFUL}.
\begin{definition}[Returning users (informal)]
\label{def:return_def}
Each user can participate in multiple batches, but within each batch she only contributes once. 
\end{definition}


% \begin{assumption}[Returning Users]
% \label{ass:return_ass}
% We assume that each user can participate in multiple batches, but within each batch she only contributes once. 
% \end{assumption}
% \sayak{Can we state this inline--not making any assumptions. Just say that each user are now allowed to participate in multiple batches.}\xingyu{I am fine with this:) but we need to emphasize that the user cannot appear twice in the same batch.}
% \sayak{Yes} \xingyu{just go ahead:)}\sayak{I will do this section and exps tomoroo} 
% \xingyu{sure, I will finish the polish for section 3, i.e, the appendix}great \xingyu{I like the current style of section 3.}\sayak{Yes, it looks good. Section 4 is very important for us. Thanks.}\xingyu{while you edit it, you can also have a double check:) haha. I give the intuition for user-level JDP, which you can easily understand. For SDP, it directly follows from composition, no fancy things.}great
% \sayak{Some equation refs are not working I see}
% \xingyu{I will fix them. You just edit your comments. Finally, I will go over to make sure there no warnings of latex.}okay


\begin{theorem}[Performance guarantees (informal)]
\label{thm:return-main}
If any user participates in at most $M_0$ rounds (i.e., $M_0$ batches by above definition), then running Algorithm~\ref{alg:BOFUL} with batchsize $B=T/M_0$, we obtain the following results for $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$, respectively. 
\xingyu{I now tend to feel that this is kind of misleading. That is we first fix $M_0$ and then tune $B$. But if $M_0=1$, we choose $B = T$?. This is not used in practice. What we used in practice is that we first fix batch size $B$ in advance, and then we chosse how to sample users. Under our assumption of returning users, we have the following guarantee. We are not trying to create batch based on how frequently users contribute. Rather, it is the server to decide how to sample users across different batches.}

(i) For any $\epsilon \!\leq\! \frac{2}{B}\sqrt{2T\log(2/\delta)}$ and $\delta \!\in\! (0,1]$, $\cP_{\text{Amp}}$ with noise levels $\sigma_1 \!=\! \sigma_2 \!=\! \frac{16\sqrt{T\log(2/\delta)(\log(5T/\delta))}}{\epsilon{B}}$ is $O(\epsilon,\delta)$-SDP, and enjoys, with high-probability, the regret bound
\begin{align*}
     \text{Reg}(T) = \widetilde{O}\left(\frac{dT}{M_0}\log T + \frac{\log^{1/2}(T/\delta)}{\epsilon^{1/2}} d^{3/4} \sqrt{M_0T}\right).
\end{align*}
(ii) For any $\epsilon \!\leq\! 15$, $\delta \!\in\! (0,1/2)$, there exist choices of parameters $g,b \!\in\! \Nat$, $p \!\in\! (0,1/2)$ depending on $B,\epsilon,\delta$ such that $\cP_{\text{Vec}}$ is $(\epsilon,\delta)$-SDP, and, enjoys the regret bound
\begin{align*}
     \text{Reg}(T) \!=\! \widetilde{O}\left(\frac{dT}{M_0}\log T \!+\!\frac{\log^{3/4}(d^2M_0/\delta)}{\epsilon^{1/2}} d^{3/4}\!\sqrt{M_0T}\right).
\end{align*}
% Let $B = O(d^{-1/6}\epsilon^{-1/3}T^{2/3}(\log(Td^2/\delta))^{1/2})$, $g = \max\{2\sqrt{B}, d, 4\}$, $p=1/4$ and 
% \begin{align*}
%     b = \frac{ 10^7\cdot \log(2/\delta)\cdot g^2 \cdot T\cdot \left(\log\left(\frac{8\cdot T(d^2+1)}{B\delta}\right)\right)^2}{\epsilon^2B^2}.
% \end{align*}
\end{theorem}
 

% \begin{theorem}[Performance guarantees (informal)]
% \label{thm:return-main}
% % Let Assumption~\ref{ass:bounded} and Assumption~\ref{ass:return_ass} hold. 
% We have the following results for $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$, respectively. 


% (i) Fix any $B \!\in\! \Nat$, $\epsilon \!\leq\! \frac{2}{B}\sqrt{2T\log(2/\delta)}$ and $\delta \!\in\! (0,1]$. Then, Algorithm~\ref{alg:BOFUL} instantiated with $\cP_{\text{Amp}}$ with noise levels $\sigma_1 \!=\! \sigma_2 \!=\! \frac{16\sqrt{T\log(2/\delta)(\log(5T/\delta))}}{\epsilon{B}}$is $O(\epsilon,\delta)$-SDP, and enjoys, with high-probability, the regret bound
% \begin{align*}
%      \text{Reg}(T) = \widetilde{O}\left(dB\log T + \frac{\log^{1/2}(T/\delta)}{\epsilon^{1/2}B^{1/2}} d^{3/4} T\right)~.
% \end{align*}

% (ii) Fix any $B\!\in\! \Nat$, any $\epsilon \!\le\! 15$, and $\delta \!\in\! (0,1/2)$. There exist choices of parameters $g,b \!\in\! \Nat$ and $p \!\in\! (0,1/2)$ depending on $B,\epsilon,\delta$ such that Algorithm~\ref{alg:BOFUL} instantiated with $\cP_{\text{Vec}}$ is $(\epsilon,\delta)$-SDP, and, enjoys, with high probability, the regret
% \begin{align*}
%      \text{Reg}(T) = \widetilde{O}\left(dB\log T +\frac{\log^{3/4}(d^2T/(B\delta))}{\epsilon^{1/2}B^{1/2}} d^{3/4}T\right).
% \end{align*}
% % Let $B = O(d^{-1/6}\epsilon^{-1/3}T^{2/3}(\log(Td^2/\delta))^{1/2})$, $g = \max\{2\sqrt{B}, d, 4\}$, $p=1/4$ and 
% % \begin{align*}
% %     b = \frac{ 10^7\cdot \log(2/\delta)\cdot g^2 \cdot T\cdot \left(\log\left(\frac{8\cdot T(d^2+1)}{B\delta}\right)\right)^2}{\epsilon^2B^2}.
% % \end{align*}
% \end{theorem}


\begin{proof}[Proof sketch]
In contrast to Section~\ref{sec:shuffleModel}, where $(\epsilon,\delta)$-SDP can guaranteed for Algorithm~\ref{alg:BOFUL} by showing each batch is $(\epsilon,\delta)$-SDP, we now need to guarantee that outputs of all the batches together have a total privacy loss of $(\epsilon,\delta)$.
This is due to the fact that now each batch can potentially operate on same set of users, and hence, one need to resort to advanced decomposition theorem. This requires scaling up the noise variance by a multiplicative factor of $O(M_0)$ at each batch, which eventually leads to the above regret bound.
\end{proof}
% \sayak{We need to write here why the noise added is bit high to guarantee privacy. Basically explain a bit where the proof is different from the previous ones. Just to get the reader know that this is achallenging setting.}\xingyu{I think what you have written is already the key:)}
% and the regret in~\eqref{eq:regret_intuition}. That is, we now need to roughly replace $\epsilon$ by $\epsilon/(\sqrt{T/B})$ in~\eqref{eq:regret_intuition}.
% \begin{remark}
% For batch size $B \!=\! O(T^{2/3})$, i.e., when each user is allowed to participate in at most $T^{1/3}$ batches, the regret of Algorithm~\ref{alg:BOFUL} is $\widetilde{O}\left( \frac{T^{2/3}}{\sqrt{\epsilon}}\right)$ for both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$ under the setting of returning users. As before, if $B$ also depends on $\epsilon$, then we can achieve a better regret $\widetilde{O}(T^{2/3}\epsilon^{-1/3})$, see Appendix~\ref{app:return}.
% \end{remark}
% \xingyu{here $B$ needs to be dependent on $\epsilon$, and hence regret is $O(T^{2/3}\epsilon^{-1/3})$ or you just consider $B = T^{2/3}$?}
% \xingyu{We can say a better $\epsilon$ dependence is possible with $B$ depending on $\epsilon$, see Appendix.}\sayak{I consider $B=T^{2/3}$}\xingyu{how about here we also show that when $B$ depends on $\epsilon$, we can have a regret $O(T^2/3\epsilon^{-1/3})$. In the following, we show that central model have the same results for both under same $M$, returning frequency somehow}\sayak{Central model does not have batch concept. People might get confused.}\xingyu{great, I was trying to say the following message: Algorithm 1 matches central model is kind of universal in that for the same different values of $M$, they continue to hold. Not just for $M = T^{1/3}$.}\sayak{I don't think regret will match for every $M$. There is a $dT/M$ term sitting in front.}
%\end{remark}
% Denoting total number of batches $M\!=\!T/B$ in Theorem~\ref{thm:return-main}, we obtain that Algorithm~\ref{alg:BOFUL} achieves regret $\widetilde{O}\left( \sqrt{TM/\epsilon}\right)$ for both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$ under the setting of returning users.
Interestingly, the privacy ($\epsilon,\delta$) dependent term in above regret bounds match the one that can be achieved in the central trust model (under the setting of returning users). Since existing work in the central model of privacy (i.e., under JDP guarantee) assume unique users~\cite{shariff2018differentially}, we first generalize it to handle returning users. This generalization can be viewed as the same as from event-level DP to user-level DP under continual observation in~\cite{dwork2010differential}, where the adjacent relation between two data streams changes from the flip of one single round to the flip of multiple rounds associated with a single user.\footnote{See Appendix~\ref{app:JDP} for formal definitions of event-level and user-level joint differential privacy (JDP).} As in standard notion of DP, one straightforward approach for converting event-level JDP to user-level JDP is to use group privacy~\cite{dwork2014algorithmic}. However, this black-box approach would blow up the terms dependent on $\delta$. To overcome this, we propose a simple modification of original (event-level) algorithm in~\citet{shariff2018differentially} so that it can handle returning users. In particular, user-level JDP can be achieved by scaling up the noise variance by a multiplicative factor of $M_0^2$, if any user participates in at most $M_0$ rounds. This follows from the fact that flipping one user now would change the $\ell_2$ sensitivity of the expanded binary-tree nodes from $O(\sqrt{\log T})$ to $O(M\sqrt{\log T})$.
This modified version enjoys the following regret guarantee.

% \sayak{State what is the modification in short.}\xingyu{This is just stated in the theorem statement, i.e., reduce $\epsilon$ to $\epsilon/M$.}\sayak{Does that mean noise level is $\frac{M^2\log T}{\epsilon^2}$}\xingyu{yes. basically reduce $\epsilon$ in previous section by a factor of $M$. see the proof sketch below.}


% this modified algorithm attains nearly the same regret bound as in Theorem~\ref{thm:return-main}  under the same value of $B$, i.e., the same number of rounds one user can contribute. 

\begin{proposition}\label{prop:JDP-return}
If any user participates in at most $M_0$ rounds, the algorithm in~\citet{shariff2018differentially}, with the above modification to handle user-level privacy, achieves the high-probability regret bound
\begin{align*}
    \text{Reg}(T) = \widetilde{O}\left(d\sqrt{T} + \sqrt{\frac{M_0T}{\epsilon}}d^{3/4} \log^{1/4} (1/\delta) \right).
\end{align*}
\end{proposition}
% with noise variance scaled up by a multiplicative factor of $M^2$ is able to achieve $(\epsilon,\delta)$-JDP (user-level) with a high-probability regret bound 
% \begin{align*}
%     \text{Reg}(T) = \widetilde{O}\left(d\sqrt{T} + \sqrt{\frac{MT}{\epsilon}}d^{3/4} \log^{1/4} (1/\delta) \right).
% \end{align*}

% \begin{proof}[Proof sketch]
% This follows from the fact that flipping one user now would change the $\ell_2$ sensitivity of the expanded binary-tree nodes from $O(\sqrt{\log T})$ to $O(M\sqrt{\log T})$. 
% \end{proof}
% \sayak{Why regret is $d^{3/4}$? ? we should give linear in $d$ term as well.}\xingyu{no, the same as previous CDP. you just check the CDP paper, you can get it. or directly look at our general result. see Lemma 3.9}\sayak{Please make the changes.}\xingyu{which change? in previous sections, you did not write any $d$ term I think.} I changed in the proposition
% \begin{remark}
% Setting $M = T^{1/3}$ yields the regret bound (i.e., $\tilde{O}(d^{5/6}T^{2/3}\epsilon^{-1/3})$) up to logarithmic factor in terms of $1/\delta$ and $T$.
% \end{remark}

\begin{remark}
Comparing Theorem~\ref{thm:return-main} and Proposition~\ref{prop:JDP-return}, we observe that the cost of privacy in the shuffle model is essentially same (upto a log factor) as in the central model under the setting of returning users.
In particular, if users participate in at most $M_0=T^{1/3}$ round, the regret is $\widetilde O\left(\frac{T^{2/3}}{\sqrt{\epsilon}}\right)$ in both shuffle and central trust models.
% For batch size $B \!=\! O(T^{2/3})$, i.e., when each user is allowed to participate in at most $T^{1/3}$ batches, the regret of Algorithm~\ref{alg:BOFUL} is $\widetilde{O}\left( \frac{T^{2/3}}{\sqrt{\epsilon}}\right)$ for both shuffle protocols $\cP_{\text{Amp}}$ and $\cP_{\text{Vec}}$ under the setting of returning users. As before, if $B$ also depends on $\epsilon$, then we can achieve a better regret $\widetilde{O}(T^{2/3}\epsilon^{-1/3})$, see Appendix~\ref{app:return}.
\end{remark}

